Scalable Ranked Preference Optimization for Text-to-Image Generation

Direct Preference Optimization (DPO) has emerged as a powerful approach to align text-to-image (T2I) models with human feedback. Unfortunately, successful application of DPO to T2I models requires a huge amount of resources to collect and label large-scale datasets, e.g., millions of generated paired images annotated with human preferences. In addition, these human preference datasets can get outdated quickly as the rapid improvements of T2I models lead to higher quality images. In this work, we investigate a scalable approach for collecting large-scale and fully synthetic datasets for DPO training. Specifically, the preferences for paired images are generated using a pre-trained reward function, eliminating the need for involving humans in the annotation process, greatly improving the dataset collection efficiency. Moreover, we demonstrate that such datasets allow averaging predictions across multiple models and collecting ranked preferences as opposed to pairwise preferences. Furthermore, we introduce RankDPO to enhance DPO-based methods using the ranking feedback. Applying RankDPO on SDXL and SD3-Medium models with our synthetically generated preference dataset "Syn-Pic" improves both prompt-following (on benchmarks like T2I-Compbench, GenEval, and DPG-Bench) and visual quality (through user studies). This pipeline presents a practical and scalable solution to develop better preference datasets to enhance the performance of text-to-image models.

==> 1_introduction.tex <==
While text-to-image (T2I) models~\citep{rombach22ldm,podell2023sdxl,dall-e3,sd3} have become widespread in the past couple of years, they still suffer from numerous shortcomings, including challenges with compositional generation~\cite{vqascore,conceptmix}, limited ability to render text and lack of spatial understanding. There have been several attempts at addressing these challenges with larger models~\citep{sd3,lit-10b}, improved datasets~\citep{schuhmann2022laion,datacomp} and superior language conditioning, but these require significantly more computational resources and do not apply to existing models. Drawing inspiration from large language models (LLMs), aligning text-to-image models with human feedback has become an important direction to enhance existing text-to-image models.

Aligning diffusion models with human feedback involves collecting large amounts of user preferences for various images generated by different models. Following the data collection process, text-to-image models can be fine-tuned by assigning higher weights to the highly preferred images~\citep{lee2023aligning,emu,richfeedback}. More recently, drawing inspiration from the success of Direct Preference Optimization (DPO)~\cite{dpo} in aligning LLMs with human feedback, there have also been similar efforts at applying this technique to text-to-image diffusion models where the goal is to improve the denoising of the more preferred images as compared to the denoising of the less preferred images~\citep{diffusiondpo,diffusionkto,mapo,spo}. However, this requires an expensive data collection process, for instance, Pick-a-Picv2~\citep{pickscore} would cost nearly \$50k following recommendations from \cite{otani2023toward}. In addition, these datasets quickly become outdated due to the rapid advancement of text-to-image models. For instance, most public datasets contain images at 512 resolution which is unsuitable for aligning modern models designed for 1024 resolution.

Alternatively, there has been a growing interest in training reward models that mimic user preferences~\citep{hps,hpsv2,imagereward,pickscore,mps}. While human preference datasets might get outdated quickly, the reward models trained on these images might generalize better to images generated by newer models. As a result, there has been a lot of interest in fine-tuning text-to-image models to maximize the scores from these reward models. It is done by generating images for various prompts, followed by backpropagating through the diffusion process to update the model parameters using reinforcement learning~\cite{ddpo,dpok,prdp,rldiffusion1,rldiffusion2} or direct backpropagation~\citep{clark2023directly,imagereward,alignprop,li2024textcraftor} to maximize the reward function. However, this process is computationally expensive due to the backpropagation through the diffusion process. Additionally, these methods suffer from ``reward hacking'' where this optimization process increases the reward scores without improving the quality of the generated images.

In this paper, we propose a scalable and cost-effective solution to the problem of aligning text-to-image diffusion models. Specifically, we investigate the efficacy of using synthetically labeled preferences in aligning text-to-image models with DPO-based techniques. While this has been studied deeply in the context of LLMs~\citep{rlaif,rlaif2}, there have been only preliminary explorations of this in the context of text-to-image models~\citep{diffusiondpo,lmmhumanannotation}, we comprehensively demonstrate the benefits of synthetically labeled preferences. First, we are able to aggregate scores from multiple reward models thereby mitigating reward overoptimization~\citep{rewardoveroptimization,reno}. Further, we are able to construct a ranking of the generated images for each prompt, unlike the conventional pairwise comparisons. While aggregating preferences across multiple labelers and constructing rankings are possible, these dramatically increase the cost of annotation compared to the minimal overhead in our case. To leverage the benefits of the richer signal from the rankings, we also introduce a ranking-enhanced DPO objective \methodName borrowing from the extensive literature on ``learning-to-rank''~\citep{burges2006learning,wang2013theoretical,wang2018lambdaloss,lipo,song2024preference}. Together, all of these techniques applied on a synthetically labeled dataset with the same prompts as Pick-a-Picv2 leads to dramatic improvements for the SDXL and SD3-Medium models in terms of prompt following and visual quality when evaluated on rigorous benchmarks such as GenEval~\citep{ghosh2023geneval}, T2I-Compbench~\citep{huang2023t2icompbench}, and DPG-Bench~\citep{ella} along with user-studies. Not only do we get better results than previous preference optimization methods (e.g. Fig.~\ref{fig:teaser}), but this also requires 5x less training time and 3x fewer images than Pick-a-Picv2. In the case of SD3-Medium (2B) which has already been optimized with 3M human preferences, we are further to get significant improvements with our synthetically labelled dataset of 240k images. Our contributions can be summarized concretely as follows:

\begin{itemize}[leftmargin=8pt,nosep]
\item We propose a synthetic labelling as a scalable and cost-effective solution to collect preference datasets for DPO fine-tuning of T2I models, eliminating the expensive human labeling costs of collecting preference datasets. 
\item We introduce \methodName~to leverage the rich ranking based annotations available from the synthetic preference labelling.
\item Applying \methodName~to SDXL and SD3-Medium achieves state-of-the-art results on several popular prompt faithfulness benchmarks while improving the visual quality of generated images. 
\end{itemize}









==> 1_introduction_v2.tex <==

While text-to-image (T2I) models~\citep{rombach22ldm,podell2023sdxl,dall-e3,sd3} have become widespread in the past couple of years, they still suffer from numerous shortcomings, including challenges with compositional generation~\citep{vqascore,conceptmix}, limited ability to render text~\citep{liu2022character}, and lacking of spatial understanding~\citep{spright}. There have been several attempts at addressing these issues with larger models~\citep{sd3,lit-10b}, improved datasets~\citep{schuhmann2022laion,datacomp}, and superior language conditioning~\citep{pixartsigma,wurstchen}, yet these works require significantly more computational resources and do not apply to existing pre-trained models. Drawing inspiration from large language models (LLMs), aligning T2I models with human feedback has become an important direction to enhance existing T2I models~\citep{liu2024alignment}.

However, training diffusion models with human feedback involves the collection of large amounts of user preferences for various images generated by different models. Following the data collection process, T2I models can be fine-tuned by assigning higher weights to the highly preferred images~\citep{lee2023aligning,emu,richfeedback}. More recently, inspired by the success of Direct Preference Optimization (DPO)~\cite{dpo} in aligning LLMs with human feedback, there have been similar efforts at applying this technique to T2I diffusion models where the goal is to improve the denoising of the more preferred images as compared to the denoising of the less preferred images~\citep{diffusiondpo,diffusionkto,mapo,spo}. Nevertheless, the data collection process is expensive. For instance, Pick-a-Picv2~\citep{pickscore} would cost nearly \$50K~\citep{otani2023toward}. In addition, these datasets quickly become outdated due to the rapid advancement of T2I models, \eg, most public datasets contain images at 512 resolution, which is unsuitable for aligning modern models designed for 1024 resolution.

Alternatively, there has been a growing interest in training reward models that mimic user preferences~\citep{hps,hpsv2,imagereward,pickscore,mps}. While human preference datasets might get outdated quickly, the reward models trained on these images might generalize better to images synthesized by newer models. As a result, there has been a lot of interest in fine-tuning T2I models to maximize the scores from these reward models. It is done by generating images for various prompts, followed by backpropagating through the diffusion process to update the model parameters using reinforcement learning~\cite{ddpo,dpok,prdp,rldiffusion1,rldiffusion2} or direct backpropagation~\citep{clark2023directly,imagereward,alignprop,li2024textcraftor} to maximize the reward function. However, this process is computationally expensive due to the backpropagation through the diffusion process. Additionally, these methods suffer from ``reward hacking'' where this optimization process increases the reward scores without improving the quality of the generated images.

In this paper, we propose a \textit{scalable} and \emph{cost-effective} solution for aligning T2I models. Specifically, we investigate the efficacy of using synthetically labeled preferences in fine-tuning T2I models with DPO-based techniques. While this has been studied in depth in the context of LLMs~\citep{rlaif,rlaif2}, there have been only preliminary explorations in the context of T2I models~\citep{diffusiondpo,lmmhumanannotation}. To this end, we develop two novel components: (a) synthetically labeled preference dataset and (b) ranking-based preference optimization. 

\textbf{Synthetically labeled preference dataset.} We generate images from different T2I models and label them with multiple human preference reward models. 
By aggregating scores from multiple reward models, we mitigate reward over-optimization~\citep{rewardoveroptimization,reno}. Unlike the conventional pairwise comparisons, we construct a ranking of the generated images for each prompt. While aggregating preferences across multiple labelers and constructing rankings are possible, these dramatically increase the annotation cost compared to the minimal overhead in our case. %

\textbf{Ranking-based preference optimization.} To leverage the benefits of the richer signal from the rankings, we introduce a ranking-enhanced DPO objective \methodName\ borrowing from the extensive literature on ``learning-to-rank''~\citep{burges2006learning,wang2013theoretical,wang2018lambdaloss,lipo,song2024preference}. It weighs the preference loss with normalized discounted cumulative gains (nDCG), enabling alignment with the preferred rankings.

Together, these techniques applied on a synthetically labeled dataset with the same prompts as Pick-a-Picv2 leads to dramatic improvements for the SDXL and SD3-Medium models in terms of prompt following and visual quality (e.g. Fig.~\ref{fig:teaser} when evaluated on rigorous benchmarks such as GenEval~\citep{ghosh2023geneval}, T2I-Compbench~\citep{huang2023t2icompbench}, and DPG-Bench~\citep{ella} along with user-studies. Not only do we get better results than previous preference optimization methods, %
but this also requires 3x fewer images than Pick-a-Picv2.
In the case of SD3-Medium (2B parameters), which has already been optimized with 3M human preferences, we are further to get significant improvements with our synthetically labeled dataset of 240K images. Our contributions can be summarized as follows:

\begin{itemize}[leftmargin=8pt,nosep]
\item We propose a synthetic labelling as a scalable and cost-effective solution to collect preference datasets for DPO fine-tuning of T2I models, eliminating the expensive human labeling costs of collecting preference datasets. 
\item We introduce \methodName~to leverage the rich ranking based annotations available from the synthetic preference labelling.
\item Applying \methodName~to SDXL and SD3-Medium achieves state-of-the-art results on several popular prompt faithfulness benchmarks while improving the visual quality of generated images. 
\end{itemize}





==> 2_related.tex <==
\myparagraph{Text-to-Image Models.} Starting from initial works employing GANs for text-to-image synthesis~\citep{reed2016generative,stackgan}, recent attempts have been centred around diffusion~\citep{ogddpm,ho2020denoising} and rectified flow~\citep{rf1,rf2,rf3} models for image and video generation. Following the success of the Stable Diffusion models~\citep{rombach22ldm,podell2023sdxl}, several improvements have been proposed, including the use of superior U-Net/transformer backbones~\citep{dit,uvit}, stronger language conditioning through superior text encoders~\citep{t5,pixartalpha,pixartsigma} and improved captions~\cite{dall-e3,sd3,spright}. In this work, we explore the efficacy of synthetically generated preferences to enhance pre-trained text-to-image model using methods based on learning from human/AI feedback.


\myparagraph{Learning from Human Preferences.} In LLMs, alignment with human preferences~\citep{ogrlfh,openairlhf,rlhf} has played a crucial role in the development of chatbots and language assistants. The paradigm of Reinforcement Learning from Human Feedback (RLHF) involved collecting large amounts of user preferences for various prompt output pairs. Following this, reward models were trained to mimic user preferences, after which reinforcement learning algorithms (e.g. PPO~\citep{ppo}, REINFORCE~\citep{reinforce,reinforcerlhf}) were used to optimize language models to maximize reward model scores. However, Direct Preference Optimization~\citep{dpo} along with similar variants~\citep{ipo,kto,orpo,simpo,lipo} emerged as a major alternative, introducing an equivalent mathematical formulation that enabled training language models directly on user preferences without requiring reward models or reinforcement learning. These insights have since been used more generally in image/video generation~\citep{diffusiondpo,diffusionkto}. Different from this line of work, we demonstrate the superior efficacy  of improving text-to-image models purely from AI feedback similar to the paradigm of Reinforcement Learning from AI Feedback (RLAIF)~\citep{rlaif,rlaif2} in LLMs.    

\myparagraph{Preference-Tuning of Image Models.} Reward models have been used effectively to fine-tune image generation models using either reinforcement learning~\citep{ddpo,dpok,prdp,rldiffusion1,rldiffusion2} or reward backpropogation~\cite{lee2023aligning,li2024textcraftor,alignprop,imagereward,clark2023directly}. However, this process is computationally expensive and has requires additional memory due to backpropogation through the sampling process and has not been successfully applied yet on larger models at 1024 resolution. As a result, following language modeling literature, DPO techniques have also been adapted to image generation~\cite{diffusiondpo,diffusionkto,spo,mapo}, thereby avoiding the expensive training objective. Differently, we demonstrate the possibility of using reward model feedback through the  denoising/preference optimization objective as a more effective solution than existing approaches for aligning text-to-image models.





==> 3_method.tex <==
In this section, we first provide an overview of diffusion models for text-to-image generation and Direct Preference Optimization for these models. Following this, we discuss the process of curating and labeling a scalable preference optimization dataset. 
\subsection{Diffusion Models}
Denoising Diffusion Probabilistic Models (DDPMs) learn to predict real data $x \sim p_{\text{data}}$ by reversing the ODE flow. Specifically, given a noisy sample $z_t = \alpha_t x + \sigma_t \epsilon$ ($\alpha_t$ and $\sigma_t$ are the SNR schedules and $\epsilon$ is the added ground-truth noise), the denoising model $\hat{{\bm{\epsilon}}}_{{\bm{\theta}}}$ parameterized by ${\bm{\theta}}$ is trained with the following objective.

\begin{equation}
     \min_{\bm{\theta}} {\mathbb{E}}_{ t \sim [1,T], \bm{\epsilon} \sim \mathcal{N}(\mathbf{0}, \mathbf{I}) } \| \bm{\epsilon} - \hat{{\bm{\epsilon}}}_{{\bm{\theta}}}( \mathbf{z}_t, \mathbf{c} ) \|^2,
\end{equation}
where $T$ is the total number of steps, and $\mathbf{c}$ is the condition signal (in the case of T2I models, the text embedding). 
\subsection{Direct Preference Optimization for Diffusion Models}
The Bradley-Terry model~\citep{bradley1952rank} defines pairwise preferences with the following formulation:
\begin{equation}\label{eq:BT}
    p_\text{BT}(\xw_0 \succ \xl_0 | \vc)=\sigma(r(\vc,\xw_0)-r(\vc,\xl_0))
\end{equation}
where $\sigma$ is the sigmoid function, $\xw_0$ is the more preferred image, $\xl_0$ is the less preferred image, and $r$ is the reward model. 

From this, \cite{dpo} showed that the following objective is equivalent to the process of explicit Reinforcement learning (e.g. PPO/Policy Gradient) with the reward model $r$. 
\begin{equation}
    L_{\text{DPO}}(\theta)\!=\!-
    \bbE_{\vc,\xw_{0},\xl_0}\left[
    \log\sigma\left(\beta \log \frac{p_{\theta}(\xw_0|\vc)}{\pref(\xw_0|\vc)}-\beta \log \frac{p_{\theta}(\xl_0|\vc)}{\pref(\xl_0|\vc)}\right)\right]
    \label{eq:dpo_loss_lang}
\end{equation}

However, in the context of diffusion models, it is not feasible to compute the likelihood of an image (i.e $p(x_0|c)$). Therefore, \cite{diffusiondpo} proposed a tractable alternative which they prove is equivalent/a minor relaxation of the original DPO objective. 

\begin{multline}
    \mathcal{L}(\theta) = - \mathbb{E}_{(\mathbf{x}^w_0, \mathbf{x}^l_0) \sim \mathcal{D}, \, t \sim \mathcal{U}(0,T), \, \mathbf{x}^w_{t} \sim q(\mathbf{x}^w_{t}|\mathbf{x}^w_0), \, \mathbf{x}^l_{t} \sim q(\mathbf{x}^l_{t}|\mathbf{x}^l_0)} \\
    \log \sigma \left( -\beta T \, \omega(\lambda_t) \left( \|\boldsymbol{\epsilon}^w - \boldsymbol{\epsilon}_\theta(\mathbf{x}_{t}^w,t)\|^2_2 - \|\boldsymbol{\epsilon}^w - \boldsymbol{\epsilon}_\text{ref}(\mathbf{x}_{t}^w,t)\|^2_2 \right. \right. \\
    \left. \left. - \left( \|\boldsymbol{\epsilon}^l - \boldsymbol{\epsilon}_\theta(\mathbf{x}_{t}^l,t)\|^2_2 - \|\boldsymbol{\epsilon}^l - \boldsymbol{\epsilon}_\text{ref}(\mathbf{x}_{t}^l,t)\|^2_2 \right) \right) \right)
\end{multline}

where $\x^*_t =  \alpha_t\x^*_0+\sigma_t\noise^*, \noise^* \sim \calN(0,I)$ is a draw from $q(\x^*_t|\x^*_0)$.
Practically, we randomly sample a timestep ($t$) compute the denoising objective at the timestep for both the winning ($x_w^t$) and the losing ($x_l^t$) sample for both the trainable and the reference models. The objective ensures that the denosing improves for the winning sample along with worsening the denoising for the losing sample. This biases the model towards generating images more like the preferred images. 

\subsection{Generating Synthetic Preferences}
However, to implement the obejctive listed out, we need access to a labelled dataset $\mathcal{D}$, which consists of paired preferences (i.e prompt, winning and losing image). Traditionally, this process requires human annotations which ends up being very expensive. Additionally, these hand-curated datasets can become outdated very quickly. Therefore, we generate images from top-performing models (e.g. SD3-Medium~\citep{sd3}, StableCascade~\citep{wurstchen}, Pixart-sigma~\citep{pixartsigma}, and SDXL) for the same prompts as Pick-a-Picv2~\citep{pickscore}. Further, our key insight is that we can label these samples using existing off-the-shelf human-preference models (e.g. HPSv2.1~\citep{hpsv2}). However, different reward models may have complementary strengths (e.g. some focus more on visual quality, others better at text-image alignment etc.). Therefore, we propose to aggregate the preferences from 5 different models (HPSv2.1~\cite{hpsv2}, MPS~\cite{mps}, PickScore~\citep{pickscore}, VQAScore~\citep{vqascore}, ImageReward~\citep{imagereward}. 
\subsection{Weighted/Ranked DPO objective}
However, unlike the traditional DPO objective which focuses on pairwise preferences, in our case, we are able to generate multiple images for the same prompt. Therefore, we would like to optimize the many-way preference at once instead of purely relying on pairwise preferences. Specifically, given a prompt $p$, and generated images $x_1, x_2, \dots, x_k$ which are ordered, we would like to ensure that the denoising for image $x_i$ is better than $x_j$ for all $i > j$. To enforce this, we draw inspiration from the Learning to Rank (LTR) literature, and repurpose the LambdaLoss by adding the nDCG weights to each sample as follows:

We first define scores $s_i$ for the $i$th sample as:
\[
s_i = \| \boldsymbol{\epsilon}_\theta(\mathbf{x}_t^i, t) - \boldsymbol{\epsilon}^i \|_2^2 - \| \boldsymbol{\epsilon}_{\text{ref}}(\mathbf{x}_t^i, t) - \boldsymbol{\epsilon}^i \|_2^2
\]
where $\boldsymbol{\epsilon}_\theta(\mathbf{x}_t^i, t)$ denotes the model’s prediction for the noisy image $\mathbf{x}_t^i$ at time step $t$, $\boldsymbol{\epsilon}^i$ is the true noise, and $\boldsymbol{\epsilon}_{\text{ref}}(\mathbf{x}_t^i, t)$ is the reference model’s prediction. This score measures how much better or worse the model's prediction is compared to the reference model.

The gain for each sample is then defined as:
\[
\phi(i) = \frac{1}{k-1} \sum_{j \neq i} \mathbb{I}(s_i > s_j)
\]
where $\phi(i)$ is the average probability that sample $i$ is preferred over all other samples $j$, computed by comparing the score $s_i$ against each other score $s_j$.

Using this, we define the gain function as:
\[
G_i = 2^{\phi(i)} - 1
\]
After computing the scores $s_i$, the images are ranked from the most preferred (lowest $s_i$) to the least preferred (highest $s_i$). The rank of each image $x_i$ is denoted by $\tau(i)$, where $\tau(i) = 1$ for the best image, $\tau(i) = 2$ for the second best, and so on.

The discount function is then defined as:
\[
D(\tau(i)) = \log(1 + \tau(i))
\]
This discount function decreases as the rank $\tau(i)$ increases, ensuring that higher-ranked images (those with a lower $\tau(i)$) have a greater influence on the final loss. The logarithmic form of the discount function smooths out the penalty differences between consecutive ranks, making the model more robust to small ranking errors, especially for lower-ranked images.

The \methodName loss is then formulated as:
\begin{multline}
\mathcal{L}_{\text{RankDPO}}(\theta) = -\mathbb{E}_{s \sim \mathcal{D}} \left[ \sum_{i > j} |G_i - G_j| \cdot \left| \frac{1}{D(\tau(i))} - \frac{1}{D(\tau(j))} \right| \right. \\
\left. \log \sigma \left( \beta \left( \| \boldsymbol{\epsilon}_\theta(\mathbf{x}_t^i, t) - \boldsymbol{\epsilon}^i \|_2^2 - \| \boldsymbol{\epsilon}_\text{ref}(\mathbf{x}_t^i, t) - \boldsymbol{\epsilon}^i \|_2^2 \right. \right. \right. \\
\left. \left. \left. - \left( \| \boldsymbol{\epsilon}_\theta(\mathbf{x}_t^j, t) - \boldsymbol{\epsilon}^j \|_2^2 - \| \boldsymbol{\epsilon}_\text{ref}(\mathbf{x}_t^j, t) - \boldsymbol{\epsilon}^j \|_2^2 \right) \right) \right) \right]
\end{multline}
where $\sigma(x)$ is the sigmoid function and $\beta$ is a temperature parameter that controls the sharpness of the preference.

This loss function encourages the model to produce images that not only satisfy pairwise preferences but also respect the overall ranking of images generated for the same prompt. By weighting the traditional DPO objective with gains and discounts derived from the ranking, we ensure that the model prioritizes the generation of higher-quality images according to the ranking, leading to more consistent improvements in both aesthetics and prompt alignment.


